Backaction suppression in levitated optomechanics using reflective boundaries

We show theoretically that the noise due to laser induced backaction acting on a small nanosphere levitated in a standing-wave trap can be considerably reduced by utilising a suitable reflective boundary. We examine the spherical mirror geometry as a case study of this backaction suppression effect, discussing the theoretical and experimental constraints. We study the effects of laser recoil directly, by analysing optical force fluctuations acting on a dipolar particle trapped at the centre of a spherical mirror. We also compute the corresponding measurement imprecision in an interferometric, shot-noise-limited position measurement, using the formalism of Fisher information flow. Our results show that the standing-wave trapping field is necessary for backaction suppression in three dimensions, and they satisfy the Heisenberg limit of detection.

==> commands.tex <==
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}
\renewcommand{\footnotesize}{\fontsize{9pt}{11pt}\selectfont}

% units in equations
\newcommand{\micron}{\text{\textmu m}}
\newcommand{\ro}{\mathbf{r}_0}

% symbols
\newcommand{\cj}{^{*}}
\newcommand{\cneeded}{\textcolor{red}{citation needed}
}
\newcommand{\sw}{(\mathbf{r}_{0},\omega)}
% enclosing environments
\newcommand{\br}[1]{\left[#1\right]}
\newcommand{\pa}[1]{\left(#1\right)}
\newcommand{\bre}[1]{\left\{#1\right\}}
\newcommand{\avg}[1]{\left\langle #1 \right\rangle}
\newcommand{\absq}[1]{\left| #1 \right|^{2}}
\newcommand{\im}[1]{\text{Im}\left[#1\right]}
\newcommand{\re}[1]{\text{Re}\left[#1\right]}



% unit vectors
\newcommand{\nx}{\hat{\mathbf{x}}}
\newcommand{\ny}{\hat{\mathbf{y}}}
\newcommand{\nz}{\hat{\mathbf{z}}}
\newcommand{\nr}{\hat{\mbf{r}}}
\newcommand{\nrr}{\hat{r}}
\newcommand{\rhat}{\hat{\mathbf{R}}}


\newcommand{\E}{\mathbf{E}}
\newcommand{\Eft}{\ft{\mathbf{E}}}
\newcommand{\B}{\mathbf{B}}
\newcommand{\Eo}{\mathbf{E}_0}
\newcommand{\Eoft}{\ft{\mathbf{E}}_0}
\newcommand{\Es}{\mathbf{E}_s}

% fluctuations
\newcommand{\dP}{\delta\mathbf{p}}
\newcommand{\dPft}{\delta\ft{\mathbf{p}}}
\newcommand{\dE}{\delta\mathbf{E}}
\newcommand{\dEft}{\delta\ft{\mathbf{E}}}
\newcommand{\polft}{\ft{\alpha}}

% frequency
\newcommand{\wo}{\omega_0}

% dyadics
\newcommand{\II}{\overline{\overline{\mathbf{I}}}}
\newcommand{\G}{\overline{\overline{\mathbf{G}}}}
\newcommand{\Go}{\overline{\overline{\mathbf{G}}}_0}
\newcommand{\Gs}{\overline{\overline{\mathbf{G}}}_s}
\newcommand{\RR}{\mathbf{R}\mathbf{R}}
\newcommand{\dyad}[1]{\overline{\overline{\mathbf{#1}}}}

% useful shortcuts
\newcommand{\dd}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ddd}[1]{\frac{\partial^{2}}{\partial^{2} #1}}
\newcommand{\ft}[1]{\tilde{#1}}
\newcommand{\atrzero}{\bigg|_{\mbf{r}_{0}=\mbf{r}'_{0}}}
\newcommand{\atrzeroo}{\bigg|_{\mbf{r}=\mbf{r}_{0}}}
\newcommand{\mbf}[1]{\mathbf{#1}}
\newcommand{\dD}[1]{\frac{d}{d #1}}
\newcommand{\df}[1]{\delta(#1)}
\newcommand{\tred}[1]{\textcolor{red}{#1}}
\newcommand{\conv}[2]{\left( #1 \ast #2 \right)(\mathbf{r}_{0},\omega) }
\newcommand{\convv}[2]{\left( #1 \ast #2 \right)(\mathbf{r}_{0}',\Omega) }
\newcommand{\corr}[2]{\avg{#1(\mbf{r}_{0},\omega)#2(\mbf{r}_{0}',\omega')}  }
\newcommand{\intconv}[3]{\int_\mathbb{R} #1(\mbf{r}_{0},\omega')#2(\mathbf{r}_{0},#3-\omega')d\omega' }

\newcommand\blankpage{%
    \null
    \thispagestyle{empty}%
    \addtocounter{page}{-1}%
    \newpage}

\renewcommand{\d}[1]{\ensuremath{\operatorname{d}\!{#1}}}

